Trisections and Ozsvath-Szabo cobordism invariants

Given a smooth, compact four-manifold $X$ viewed as a cobordism from the empty set to its connected boundary, we demonstrate how to use the data of a trisection map $\pi:X^{4} \to \mathbb{D}^{2}$ to compute the induced cobordism maps on Heegaard Floer homology associated to $X$.

==> Relative-Invariants/Mayer-Vietoris-Strategy.tex <==
\subsection{A Mayer-Vietoris strategy}
\label{subsec:MV-strategy}

For a closed $4$-manifold $X$ with $b_{2}^{+}(X) \geq 2$ Ozsv\'ath and Szab\'o defined a map
\[
\Phi_{X}: \spinc(X) \to \F
\]
It is common to write $\Phi_{X, \ss}$ for the value of $\Phi_{X}$ on $\ss$. The map $\Phi_{X}$ is referred to as the \emph{mixed invariant} of $X$, because it intertwines $HF^{+}$ and $HF^{-}$.

The map $\Phi_{X}$ is defined by picking a connected, codimension one submanifold $N \subset X$ that cuts $X$ into two pieces, $W_{1}$ and $W_{2}$, such that $b_{2}^{+}(W_{i}) > 0$, and such that the restriction map
\[
H^{2}(X) \to H^{2}(W_{1}) \oplus H^{2}(W_{2})
\]
is an injection. Such a three-manifold $N$ is called an \emph{admissible cut}. If we view $W_{1}$ as a cobordism from $S^{3}$ to $N$, and $W_{2}$ as a cobordism from $N$ to $S^{3}$ the maps $F^{\infty}_{W_{1}, \ss|_{W_{1}}}$ and $F^{\infty}_{W_{2}, \ss|_{W_{2}}}$ vanish \cite[Lemma 8.2]{ozsvath2006holomorphic}. Consequently, the image of $F^{-}_{W_{1}, \ss|_{W_{1}}}$ lands in $HF^{-}_{\reduced}(N, \ss|_{N})$ and the map $F^{+}_{W_{2}, \ss|_{W_{2}}}$ factors through $HF^{+}_{\reduced}(N, \ss|_{N})$. Finally, using the isomorphism between $HF^{-}_{\reduced}(N, \ss|_{N})$ and $HF^{+}_{\reduced}(N, \ss|_{N})$ via $\delta$, one arrives at the following diagram 

\begin{figure}[ht]
    \centering
    \begin{tikzcd}
                               &                                          &                                  & HF^{-}(S^{3}) \ar{d}{F^{-}_{W_{1}, \ss|_{W_{1}}}} \arrow[dashed]{dl} \\
    HF^{+}(N, \ss|_{N}) \ar{d}[swap]{F^{+}_{W_{2}, \ss|_{W_{2}}}} \ar{r} & HF^{+}_{\reduced}(N, \ss|_{N}) \arrow[dashed]{dl} \ar{r}{\delta} & HF^{-}_{\reduced}(N, \ss|_{N}) \ar{r} & HF^{-}(N, \ss|_{N}) \\
    HF^{+}(S^{3})              &                                          &                                  & 
    \end{tikzcd}
    \label{fig:mixed}
\end{figure}

Recall that the Floer homology groups of $S^{3}$ can be computed as
\[
HF^{-}_{k}(S^{3}) = \begin{cases}
\F & \text{if $k$ is even and $k \leq -2$} \\
0 & \text{else}
\end{cases}\qquad HF^{+}_{k}(S^{3}) = \begin{cases}
\F & \text{if $k$ is even and $k \geq 0$} \\
0 & \text{else}
\end{cases}
\]
The invariant $\Phi_{X, \ss}$ is defined as the coefficient of the bottom-graded generator $\Theta_{+}$ of $HF^{+}_{(0)}(S^{3})$ in the expression
\begin{equation}
    \label{eq:mixed-map}
    \Big( F^{+}_{W_{2}, \ss|_{W_{2}}} \circ \delta^{-1} \circ F^{-}_{W_{1}, \ss|W_{1}} \Big) (\Theta_{-})
\end{equation}
where $\Theta_{-}$ denotes the top-graded generator of $HF^{-}_{(-2)}(S^{3}) \cong \F$. Ozsv\'ath and Szab\'o prove that this is independent of the choices made (for example, the choice of admissable cut). 

An equivalent formulation is to utilize the pairing on Heegaard Floer homology defined on $CF^{\infty}(Y, w, \ss)$ via
\begin{equation}
    \label{eq:pairing}
    \langle \cdot, \cdot \rangle: CF^{\infty}(Y,w,\ss) \otimes CF^{\infty}(-Y,w,\overline{\ss}) \to \F \qquad \langle [\xx, i], [\yy, j] \rangle = \begin{cases}
    1 & \text{ if $i + j = -1$ and $\xx = \yy$} \\
    0 & \text{else}
    \end{cases}
\end{equation}

This pairing descends to one on $\langle \cdot, \cdot \rangle : HF^{+}_{\reduced}(Y, w, \ss) \otimes HF^{-}_{\reduced}(-Y, w, \overline{\ss}) \to \F$ \cite[Section 5.1]{ozsvath2006holomorphic}. Using this pairing, we can alternatively define $\Phi_{X, \ss}$ via the duality properties of Heegaard Floer homology. Namely, instead of viewing $W_{2}$ as a cobordism from $N$ to $S^{3}$, we can `turn $W_{2}$ around', and view it as a cobordism $\overline{W}_{2}: -S^{3} \to -N$, where $-N$ denotes the three-manifold $N$ with its orientation reversed. In \cite[Section 5.1]{ozsvath2006holomorphic}, Ozsv\'ath and Szab\'o show that the maps
\[
F^{-}_{\overline{W}_{2}, \overline{\ss}} \qquad \text{and} \qquad F^{+}_{W_{2}, \ss}
\]
are adjoint to each other with respect to $\langle \cdot, \cdot \rangle$. 

Following \cite{jabuka2008product}, we make the following definition.

\begin{definition}
\label{def:Relative-Invariant}
For a smooth, compact, connected, oriented $\spinc$ four-manifold $(W, \ss)$ with connected boundary $\partial W = Y$, we define the \emph{relative invariant} of $(W, \ss)$ to be the image of $\Theta_{-} \in HF^{-}_{(-2)}(S^{3})$ under the cobordism map
    \begin{figure}[ht]
        \centering
        \begin{tikzcd}[row sep = 0.01in]
        HF^{-}(S^{3}) \ar{r}{F^{-}_{W, \ss}} &  HF^{-}(Y, \ss|_{Y}) \\
        \Theta_{-} \ar[mapsto]{r} & \Psi_{W, \ss}
        \end{tikzcd}
        \label{fig:Defn-Relative-Invariant}
    \end{figure}
where we view $W$ as a cobordism from $S^{3}$ to $Y$ after removing a small four-ball from $W$.
\end{definition}

It follows from the discussion above that if $X$ is a four-manifold with $b_{2}^{+}(X) \geq 2$ and is decomposed into two pieces as above, then the mixed invariants can be recovered as
\begin{equation}
    \label{eq:MV-Mixed}
    \Phi_{X, \ss} = \langle \delta^{-1} \Psi_{W_{1}, \ss|W_{1}}, \Psi_{\overline{W}_{2}, \overline{\ss}|_{\overline{W}_{2}}} \rangle
\end{equation}

With this strategy in mind, our main focus in the upcoming sections will be on computing the relative invariants from a (relative) trisection.
